Zero-Resource Hallucination Prevention for Large Language Models

The prevalent use of large language models (LLMs) in various domains has drawn attention to the issue of "hallucination," which refers to instances where LLMs generate factually inaccurate or ungrounded information. Existing techniques for hallucination detection in language assistants rely on intricate fuzzy, specific free-language-based chain of thought (CoT) techniques or parameter-based methods that suffer from interpretability issues. Additionally, the methods that identify hallucinations post-generation could not prevent their occurrence and suffer from inconsistent performance due to the influence of the instruction format and model style. In this paper, we introduce a novel pre-detection self-evaluation technique, referred to as SELF-FAMILIARITY, which focuses on evaluating the model's familiarity with the concepts present in the input instruction and withholding the generation of response in case of unfamiliar concepts. This approach emulates the human ability to refrain from responding to unfamiliar topics, thus reducing hallucinations. We validate SELF-FAMILIARITY across four different large language models, demonstrating consistently superior performance compared to existing techniques. Our findings propose a significant shift towards preemptive strategies for hallucination mitigation in LLM assistants, promising improvements in reliability, applicability, and interpretability.

==> Files/adversarial.tex <==
\section{Text Adversarial}
\subsection{Related Concepts}
\subsubsection{Basic Logic}
Locate the target words or sentences, then apply gradient search or similar approaches to flip the prediction results. So we can borrow the methods for locating import words or sentences. 

The logic of text adversarial attack: finding machine believed important parts then replace it with something human does not think very different.

The logic of our goal: finding machine believed unimportant parts while human does not think so. Or, finding important sentences as the pseudo-ground-truth for text summarizing.

\subsubsection{Core Problems} 
how to define a salience score for model and for human?

The methods of text adversarial attack for salience scores: Rely on downstream classifiers. Remove the target words or sentence, and compare the change of the prediction results. Bigger the change, Higher the salience score.

For us: we can remove or replace the words and sentence then, compare the difference of the following generated sentences with certain metrics like R1 R2 scores. Bigger the change, higher the machine salience score. For human salience score, it may be more difficult to define. User can assign it at first or through entity detection methods.

\subsection{Solution}
With the \textbf{model salience scores} and \textbf{human salience scores}, we can define a \textbf{hallucination score} by comparing the difference. 
\begin{equation}
    HallucinationScore = \sum w_t(Sali^{human}_t - Sali^{model}_t) 
\end{equation}
$Sali^{human}_t$ and $Sali^{model}_t$ are the salience scores for the critical words (concepts).

For text summarizing, the \textbf{high salience sentence} will be regarded as the pseudo labels.
We can use Prompt+probability to define sentence salience score:
\begin{equation}
    SummarySCORE = \sum w_tlog p(y_t|y<t,x+pro,\theta)
\end{equation}
Giving the test sentence $x$ and prompt $pro$, we calculate the probability for generating the remaining sentences. $w_t$ is the weight, which we can use knowledge or entity to make important words or concepts have bigger contribution.
\subsubsection{Word Salience}
\begin{itemize}
    \item Replace: Replace word with "UNKNOW" then compare the change of prediction scores~\cite{ren2019generating}.
    \item Integrated Gradient~\cite{sundararajan2017axiomatic}: gradually considering the gradient contribution of the word.
\end{itemize}


\subsubsection{Sentence Difference Score}
\begin{itemize}
    \item FactCC~\cite{kryscinski2019evaluating}: a supervised factual consistency checking model
    \item BERTScore~\cite{zhang2019bertscore} aggregates similarity scores between the BERT contextual embedding of tokens in candidate and reference sentences.
    \item BARTScore~\cite{yuan2021bartscore} evaluates text using probabilities from force-decoding with a BART
model 
    \item CTC~\cite{deng2021compression} measures the average token-level alignment of the generated text w.r.t the grounding text using a BERT sequence tagging model.
\end{itemize}
\subsection{Choose One}
\subsubsection{Hallucination}
\begin{itemize}
    \item Pros: 1. Probably a better topic for AAAI. 2. We can avoid comparison with Prompt Programming LLM methods by emphasizing the expert domains: e.g. a lanague model fine-tuned on Legal QA, is not able to perform self-checking by NL instructions.
    \item Cons: 1. need to create evaluation data by ourselves.
    \item steps: deploy a local model e.g. LAMA to test. Set up examples, try it on GPT-3 and 4.
\end{itemize}
\subsubsection{Zero-shot Summarization}
\begin{itemize}
    \item Pros: 1. A relatively known topic.
    \item Cons: 1. May need to compare with the LLM prompt programming methods and is hard to guarantee better than chatgpt+prompts on zero-shot setting.
    \item steps: Set-up recent few-shot baselines and datasets. Find a suitable LM to calcuate sentence salience scores. Apply the pesudo labels.
\end{itemize}
\subsection{Word Salience For Text Generation}
\begin{itemize}
    \item The evaluation should be robust to position change. 
    \item The influence of target words can appear in any generated sub-sequence.
    \item The choice of prompt. For example, adding the detail requirement to the prompt maybe helpful to maximize the influence of the key words.
    \item should ignore the stop words difference.
    \item should ignore the first inference results.
\end{itemize}
\subsection{Significance Score}
Change the key words, then use the decoding probability of the original output sequence to estimate the influence.
\begin{equation}
    x = [x_1,\cdots,KEY, x_n]
\end{equation}
\begin{equation}
    [y_1,\cdots,y_n] = Decode(x, \theta)
\end{equation}
\begin{equation}
    p_t = p(y_t|y<t, x, \theta)
\end{equation}
\begin{equation}
    \hat{x} = [x_1,\cdots,UNK, x_n]
\end{equation}
\begin{equation}
    \hat{p}_t = p(y_t|y<t, \hat{x}, \theta)
\end{equation}
\begin{equation}
    s_{sig} = \sum w_t p_t|p_t-\hat{p}_t|
\end{equation}
Where $w_t=0$ if $y_t$ is a stop word or a $KEY$ word.
The purpose of the familiar score is to evaluate how the answer is related to the input concept.
If the score is low, it is likely to indicate a hallucination.
In addition, if sub-concepts are significantly higher than the over-all concept. It is also likely to indicate a hallucination.
\subsection{Familiar Score}
Under the prompt context, let the model predict the $KEY$ word.
\begin{equation}
    \hat{x} = [x_1,\cdots,UNK, x_n]
\end{equation}
\begin{equation}
    \hat{x}_p = [The\ UNK\ is]
\end{equation}
\begin{equation}
    [p_1,\cdots, p_m] = P(\hat{x}+\hat{x}_p, \theta)
\end{equation}
\begin{equation}
    \mu = Mean(p_1,\cdots, p_m)
\end{equation}
\begin{equation}
    \sigma = STD(p_1,\cdots, p_m)
\end{equation}
\begin{equation}
    s_{fim} = \frac{p_{key}}{e^{\sigma}}
\end{equation}
The purpose of the familiar score is to evaluate how familiar is the model to the input concept.
If the score is low, it is likely to indicate a hallucination.


The metrics should be multi-modal. First is the significance score for evaluating the contribution of the key concepts to the response.
The second is the familiar score, which measures how familiar the complicated concepts are to the models.
If one of the two metrics is below the standard, we can make sure that the answer is highly in-confidential.
\subsection{Back Score}
Current problem. The idea of the familiar score is not suitable for the decoder model.
Since decoder models do not contain the [MASK] language prediction task. Using is, means such words are not a very strict hint.
For example, "is a", "is a concept of", "is talking about". It is hard to guarantee the words after the hint words are what we want.
Thus the estimated probability of the target words is often zero.

Instead of such strict estimation. If we let the model freely generate the following sentences, we can still find the target words.
Thus for the new solution, using constraints to force the model to generate the guess with the target words. Then, compared the sequence probability with the maximum greedy search result.
\section{Previous Methods}
Existing hallucination detection methods majorly focus on post-detection. The methods focus on the classification of hallucination outputs.
Based on the methods applied, they can be classified into two major groups. The first group of methods focuses on self-checking, using the original models' parameters and outcomes, majorly the token probability distribution to estimate the hallucination level. The core idea is to generate the response multiple times and compare the difference between the responses.

The second group of methods relies on external tools, e.g., another LLM to evaluate the response with Chain of Thoughts (CoT) or additional retrieval results from the search engine or knowledge base. This kind of method is very limited. Thus the procedure is often designed for one specific response and is not able to address a general format. For example, contradiction detection, fairness detection, and consistency detection. One of the other problems is that the dataset is often both generated and evaluated by the same LLM ChatGPT. As a result, it can be biased.
\section{Existing Datasets}
The current datasets for hallucination detection only consider the post-detection. The prompt and response are given, the goal of the target model is to choose the correct response or judge if the responses are wrong. Those datasets are limited since they did not take into account the difference between different LLMs. Different LLMs can have different background knowledge, and the hallucination response to one model can be easily recognized by another model. Second, even if the model can classify one specific hallucination response, it cannot guarantee that the model won't generate a different hallucination response. And most of the methods only evaluate the ChatGPT, and the obtained results are very biased.
\section{Our Method}
\subsection{Hypothesis}
If the model is familiar with a specific concept, the map between the concept and the generated response that is based on the concept should be a One-to-One Mapping.
\begin{equation}
    y = f(x|\theta, prompt)
\end{equation}
Here, the $prompt$ and the LLM $\theta$ make up the mapping function and the concept $x$ and the response $y$ are the input and output of the function.
\subsection{Finding relation \textbf{$x\Rightarrow y$}}
\begin{equation}
    [p_1,\cdots,p_n] = GreedyDecode(f(x|\theta, prompt))
\end{equation}
\begin{equation}
    [\hat{p}_1,\cdots,\hat{p}_n] = ForceDecode(f(unk|\theta, prompt, y))
\end{equation}
By replacing $x$ with $unk$, compare the output probability sequence of $y$. If the sequence changes a little, we can conclude that $x$ has a small influence on $y$. Thus the generated response is general, not based on $x$. $x$ can lead to multiple $y$. We can conclude that the model is not familiar with the concept $x$.
\subsection{Finding relation \textbf{$y\Rightarrow x$}}
Let $f()$ be \emph{"explain the $x$"} and we can use \emph{"$y$ is explaining what concept"} as the $f^{-1}()$.
\begin{equation}
    [p_1^\prime,\cdots,p_m^\prime] = ConsBeamDecode(f(y|\theta, prompt^{-1}, x))
\end{equation}
$[p_1^\prime,\cdots,p_m^\prime]$ is the best probability sequence of the $ConsBeamDecode$. $ConsBeamDecode$ means we use beam search to force the model to return a response that must contain $x$. We can use the $[p_1^\prime,\cdots,p_m^\prime]$ to estimate the score of the response. If the score is low, means the generated $y$ is not strictly linked to the concept $x$. $y$ can lead to multiple $x$. Hence, we can also conclude that the model is not familiar with the concept $x$.
\section{Dataset Construction}
\subsection{Fictional Concepts}
Using the prompt “Make up some fictional \{domain\} concepts”. We can easily obtain many cases, and we can send them back to ChatGPT if they trigger the protection response, we can make sure such concepts are not existing.
\subsection{New Concepts or Events}
For example, any events or concepts that happened or developed later than 2022 are basically unknown to the current LLMs.
\subsection{Culture Transfer}
Using the concepts from a low-resource language.
\subsection{Construction}
With the concepts, feed them into several pre-designed templates to generate a query.
\begin{itemize}
    \item What is the meaning of \{concept\} (catchphrase)?
    \item What is the impact of the \{concept\} (event)?
    \item What diseases can \{concept\} be applied to (medical)?
    \item What is the symptom of \{concept\} (disease)?
    \item What can we learn from the \{concept\} (business/law cases)?3
\end{itemize}

\subsection{Existing hallucination datasets}
\begin{itemize}
    \item 
\end{itemize}
\subsection{Limitations}
\begin{itemize}
    \item Focusing on single topics.
    \item Highly relies on ChatGPT, using ChatGPT to generate and evaluate at the same time. 
    \item Do not reflect the essence of the hallucination.
\end{itemize}
\subsection{Our focus}
\begin{itemize}
    \item Self-evaluation
    \item Reflect the essence of the hallucination. Inadequacy of the knowledge.
    \item A balanced evaluation dataset that can be applied to different models.
    \item how to craft it?
    
\end{itemize}
\subsection{Metrics}


==> Files/data.tex <==
%Move to experiment



\section{Dataset}
\begin{table}[]
\centering
\caption{Statics information of the dataset.}
\label{tab:dataset}
\begin{tabular}{ll}
\hline
\multicolumn{2}{c}{Concept-7}                            \\ \hline
\multicolumn{1}{l|}{\# of basic concepts}          & 192 \\
\multicolumn{1}{l|}{\# of basic questions}           & 451 \\
\multicolumn{1}{l|}{\# of test concepts}           & 180 \\
\multicolumn{1}{l|}{\# of real test concepts}      & 106 \\
\multicolumn{1}{l|}{\# of fictional test concepts} & 74  \\
\multicolumn{1}{l|}{\# of test questions}            & 515 \\ \hline
\end{tabular}
\end{table}

\cx{move both data and task to the experiment section}
 Most existing datasets predominantly concentrate on the classification of hallucinatory responses. To effectively evaluate our method, we introduce the {\data} dataset, which places an emphasis on the classification of potential hallucinatory instructions. This dataset encompasses 192 foundational concepts and 180 test concepts sourced from seven expert domains. A comprehensive overview of the dataset is displayed in Table~\ref{tab:dataset}.

\subsection{Tasks}
To assess the performance of our proposed {\method} in counteracting hallucinations, we establish two experimental scenarios. For both, the domain of the instruction is explicitly supplied to mitigate potential issues with polysemy, and the algorithms are required to judge if the instruction is a hallucinatory instruction. Instructions comprising unfamiliar concepts are deemed to be hallucinatory instructions. 

\noindent \textbf{Concept-level} This scenario aims to appraise a model's understanding of a particular concept. A standard instruction, \textit{"Explain the \{concept\} in the \{domain\} domain within one short paragraph."} is uniformly applied to all concepts. 

\noindent \textbf{General-level} For each concept, we generate three questions to serve as target instructions for evaluating the algorithms. The algorithms are required to ascertain the hallucination level of these instructions, thereby mimicking real-world applications.

\subsection{Dataset Creation}
In the subsequent section, we delve into the specifics of dataset construction.

\noindent \textbf{Concept Selection}
Initially, we select 192 fundamental concepts, guided by the popular pages on Wikipedia\footnote{\url{https://en.wikipedia.org/wiki/Wikipedia:Popular_pages}} and domain diversity. These concepts are considered universally known for all language models and serve as a benchmark for the classification of familiar concepts.
For the test concepts, we choose 106 concepts from seven expert domains: Legal, Medical, Finance, Music, Art, Physics, and History. To maintain a balanced proportion between familiar and unfamiliar concepts, we fabricate 74 fictional concepts built upon real ones. As these fictional concepts don't exist, they're inherently deemed unfamiliar to all language models. However, as the training sources vary for each language model, it is necessary to annotate familiarity scores for the real concepts for each model under test.

\noindent \textbf{Familiarity Annotation}
To assign familiarity scores, we propose a comparison between a crafted gold-standard explanation of concepts and each language model's generated explanation. This familiarity assessment is conducted automatically via GPT-4. We instruct GPT-4 to provide a familiarity score for the model in relation to the concept on a scale of "1-9", as described in Appendix~\ref{app:gpt4-eval}. A threshold of "5" is chosen; concepts with a score exceeding "5" are deemed familiar, whereas those scoring less are deemed unfamiliar. Concepts scoring exactly "5" are manually reviewed for final labeling. Additionally, we employ Amazon Mechanical Turk\footnote{\url{https://www.mturk.com/}} to gather pure human annotation results for the highest-performing model as a secondary evaluation method, ensuring the effectiveness of the GPT-4 annotated results. For human-annotated results, we have three different annotators for each concept and the final label is decided based on the average score. If the average score happens to be “5”, a majority vote is applied to decide the label.

\noindent \textbf{Generating General-level Instructions}
To replicate general conversational scenarios, we use a prompt (as shown in Appendix~\ref{}) to generate three related questions for each concept via GPT-3.5. This includes two open-ended questions and one yes-or-no question. We subsequently discard questions that fail to mention the original concept to maintain strong relevance. Any questions that integrate previously unfamiliar concepts are marked and classified under the "hallucinatory instruction" category.

==> Files/intro.tex <==

%\textcolor{red}{Junyu, there are some arxiv papers on this topic, such as this one \url{https://arxiv.org/abs/2306.16564} \url{https://arxiv.org/abs/2305.11747} \url{https://arxiv.org/abs/2303.08896} . I think we need to mention and compare with some of these newer approachers to enhance our baselines. Some discussion we could refer to \url{https://arxiv.org/abs/2305.14552} }

%Intro
%Related work summarization
%limitaiton
%techinial challenge
%proposed method

\section{Introduction}

\cx{perhaps we only need a brief summary here.  - The widespread adoption of Large Language Models (LLMs) has generated significant interest in their application across diverse use cases, e.g., healthcare and legal. However, a major challenge hindering their full potential is the issue of hallucination, where the models produce inaccurate or fabricated information, leading to a substantial gap in their reliability and trustworthiness.}
The advent of large language models (LLMs) has enabled the application of various language assistants, such as ChatGPT, Copilot, and Bing, in a multitude of settings. However, this widespread use of large language models has rekindled attention to the issue of hallucination. In the context of language models, ``hallucination'' refers to instances where the model generates ungrounded or factually inaccurate information, straying from the provided input or instructions as shown in Fig.~\ref{fig:example}.
Gaining a deeper understanding of these hallucinations and devising effective management strategies can enhance the accuracy of language model outputs, reducing the likelihood of generating misleading or false information. This is not only pivotal for improving overall model performance but is also a matter of safety and ethics, particularly when AI is applied in sensitive domains such as news generation, medical advisory services, or legal counsel.


\begin{figure}[h]
\centering
\includegraphics[width=\linewidth,natwidth=610,natheight=642]{Images/example.pdf}
\caption{A hallucination example. \textcolor{red}{Red} color indicates the incorrect information. }
% \url{https://chat.openai.com/share/6db6c4a9-2d50-48ec-ad78-b67d2de16df4}
\label{fig:example}
\end{figure}

\cx{Language model development has seen significant advancements, however, the problem of hallucination and ways to prevent it in language assistants have been largely overlooked until recently. Researchers have started addressing this issue, and the current hallucination detection methods fall into the following categories:} 
\cx{Summarize the existing approaches and provide reference here: (1) chain-of-thought methods, (2) parameter-based methods}
Despite significant advancements in language model development over the past decades, the issue of hallucination and the exploration of potential prevention methods on language assistants have largely been overlooked. It is only recently that researchers have begun to shift their focus toward this pressing issue. In summary, the current hallucination detection methods can be classified into two categories and each category has its' own limitation.


\cx{summarize the open challenges below.}

\begin{itemize}
    \item \textbf{Lack of accurate result and universality}. The first category of methods~\cite{gou2023critic,zhang2023mitigating,min2023factscore,zhang2023interpretable, mundler2023self} hinges on a third-party knowledge base, combined with the Chain of Thought (CoT) technique, to identify and rectify potential hallucination responses. Specifically, background information is initially obtained via a search engine or database. Subsequently, this information is input into the language model through a specially crafted prompt to perform a CoT evaluation of the generated response.
While the CoT technique can frequently produce high-quality results accompanied by comprehensive explanations, it also carries significant limitations. Primarily, the evaluation output tends to be in a free text format, thus is hard to obtain an accurate result and it complicates the development of a precise control system \cx{I dont quite follow why "free text form" indicates "hard to obtain accurate results"}.
Secondly, CoT methods place substantial reliance on the intrinsic inferencing ability of models, and only a handful of large language models possess such capabilities. As a result, not every large language model is able to perform it well.

\item \textbf{Lack of interpretability}. \cx{if we cannot demonstrate strong interpretability with the proposed method, we should not point out this challenge.  }
Consequently, some researchers have shifted their focus toward parameter-based methodologies~\cite{manakul2023selfcheckgpt,min2023factscore}. For such methods, there is no reliance on a third-party model or knowledge, nor are there specific demands for the prompt format. Therefore, parameter-based methods lend themselves more readily to open-ended conversations.
Nonetheless, parameter-based typically depends on the response sequence probability information (e.g., perplexity, sampling from probability sequence) of the language models. This information does not directly correlate with the veracity of the generated response. Therefore, parameter-based methods often lack interpretability and exhibit subpar performance compared to CoT techniques.
\item \textbf{Lack of reliability and robustness}: \cx{if the proposed model does not have any specific design to handle noise, we should not point out this challenge either.  }
Finally, all the aforementioned methods concentrate on the post-detection of hallucination responses. These approaches can only determine whether a response is a hallucination, without the ability to prevent the generation of such responses in the future, which makes it less reliable. Additionally, as the output is highly dependent on the instruction, thus all the current methods do not maintain robust performance in open conversation scenarios, making it challenging to establish a threshold to discern hallucination responses. For instance, 'yes' or 'no' queries often elicit very brief response sequences. Hence, the metrics derived are frequently divergent from those derived from lengthier response sequences. Therefore, a more proactive, preventative approach to hallucination responses is highly desirable for the practical and efficient application of AI language assistants.
\end{itemize}

\cx{I think the possible angles might include : (1) post-hoc vs. proactive (2) dependence on expert knowledge - costly and limited vs. automate and data-driven. (3) some other minor angles if there are experiments to demonstrate. }


In stark contrast, humans excel at preventing hallucinations and conducting self-evaluations, largely due to our awareness of what we know and what we don't. As such, individuals with wisdom tend to refrain from passing judgment on unfamiliar concepts or topics to avoid incorrect responses. Large language models could also gain significant advantages by adopting a similar approach.

\cx{for the paper title, model name, name of this familiarity score, we might need to discuss and see if there are better alternatives.  }
To this end, we propose a novel zero-shot pre-detection technique, which we refer to as {\method}.  
\cx{before the discussion on its novelty. please summarize the proposed method, with focus on : the technical contribution, the workflow, the input and output }
\jl{***See intro_new.tex***}
Unlike post-detection methodologies, {\method} assesses the model's familiarity with the concepts introduced in the input instruction to stop the hallucination response. Thus, it is more reliable and robust. In addition {\method} amalgamates the advantages of the CoT technique and parameter-based methods, therefore circumventing their limitations while preserving their benefits. 
We evaluated our method across four large language models, each with different base frameworks and training data. The proposed {\method} consistently demonstrated state-of-the-art performance on all models when compared to other methods, thereby showing its potential for improving the reliability and relevance of responses generated by these models.

In summary, we have the following contributions:
\begin{itemize}
\item We propose a novel pre-detection zero-shot methodology, {\method}, which evaluates the model's familiarity with the concepts of the input instruction to prevent the generation of hallucinated responses.
\item We propose a hallucination instruction pre-detection dataset {\data} with concepts and instructions from 7 expert domains and an automatic evaluation method making it can easily be applied to different language models.
\item We demonstrate the practical application of the {\method} technique across a diverse range of large language models with different base frameworks and training data. The proposed methodology consistently exhibits superior performance over existing zero-shot methods, offering promising improvements in the reliability and applicability of AI language models. In addition, our proposed method also offers great interpretability. 
\end{itemize}


==> Files/temp.tex <==
\section{Previous Methods}

Existing methods for hallucination detection primarily focus on post-detection and the classification of hallucination outputs.

These methods can be classified into two major groups based on the approaches employed. The first group of methods focuses on self-checking, wherein the original model's parameters and outcomes, particularly the token probability distribution, are used to estimate the level of hallucination. The fundamental idea is to generate the response multiple times and compare the differences between these responses.

The second group of methods relies on external tools, such as another Language Model (LM), to evaluate the response using techniques like Chain of Thoughts (CoT) or by incorporating additional retrieval results from search engines or knowledge bases. However, these methods are often limited in scope, as they are designed for specific responses and may not address a general format. For instance, they may struggle with detecting contradictions, fairness issues, or inconsistencies. Another challenge with these methods is that the datasets used for training and evaluation are often generated and evaluated by the same LM, ChatGPT, which can introduce biases.

\section{Existing Datasets}

Current datasets for hallucination detection primarily focus on post-detection scenarios. In these datasets, the prompt and response are provided, and the target model's objective is to choose the correct response or determine whether the responses are incorrect. However, these datasets have limitations. Firstly, they do not consider the variations between different LMs. Different LMs may possess varying background knowledge, allowing one model to easily recognize a hallucination response that another model might miss. Secondly, even if a model can successfully classify a specific hallucination response, it does not guarantee that the model will not generate a different hallucination response in the future. Additionally, most of the existing methods only evaluate the performance of ChatGPT, leading to biased results.
\section{Our Method}
Instead of post-detection, our method focuses on the prevention of hallucination response by estimating the concept of familiarity with the queries and preventing the model to generate responses to unfamiliar topics to avoid hallucination. 
\subsection{Hypothesis}
If the model is familiar with a specific concept, the map between the concept and the generated response based on that concept should exhibit a One-to-One Mapping. By properly choosing the prompts, we can find such mappings.

\begin{equation}
y = f(x|\theta, \text{prompt})
\end{equation}

Here, the $x$ represents the concept and the $y$ represents the response, while $\text{prompt}$ and LLM $\theta$ constitute the mapping function.

\subsection{Finding relation $x\Rightarrow y$}
\begin{equation}
[p_1,\cdots,p_n] = \text{GreedyDecode}(f(x|\theta, \text{prompt}))
\end{equation}

\begin{equation}
[\hat{p}_1,\cdots,\hat{p}_n] = \text{ForceDecode}(f(\text{unk}|\theta, \text{prompt}, y))
\end{equation}

By replacing $x$ with $\text{unk}$, we compare the output probability sequence of $y$. If the sequence changes only slightly, we can conclude that $x$ has a minimal influence on $y$. Consequently, the generated response is general and not based on $x$. Additionally, $x$ can lead to multiple $y$ values. Thus, we can infer that the model is not familiar with the concept $x$.

\subsection{Finding relation $y\Rightarrow x$}
Let $f()$ represent "explain the concept $x$", and we can use "$y$ is explaining what concept" as the inverse function $f^{-1}()$.

\begin{equation}
[p_1^\prime,\cdots,p_m^\prime] = \text{ConsBeamDecode}(f(y|\theta, \text{prompt}^{-1}, x))
\end{equation}

$[p_1^\prime,\cdots,p_m^\prime]$ represents the best probability sequence obtained through the  \text{ConsBeamDecode} process. \text{ConsBeamDecode} uses beam search to force the model to generate a response that must contain $x$. We can use $[p_1^\prime,\cdots,p_m^\prime]$ to estimate the score of the response. If the score is low, it indicates that the generated $y$ is not strongly related to the concept $x$. This implies that $y$ can lead to multiple $x$ values. Consequently, we can conclude that the model is not familiar with the concept $x$.

\section{Dataset Construction}
Since we focus on prevention, the goal of the dataset is to include queries that will lead to hallucination responses. In our setting, it equals the queries that contain unfamiliar concepts to the tested LMs. The task of the dataset is to classify the queries into hallucination queries and normal queries based on the target language model.
\subsection{Fictional Concepts}
Using the prompt "Create fictional {domain} concepts," we can easily generate numerous cases. We can send these cases back to ChatGPT and verify if they trigger a protection response. This allows us to ensure that such concepts do not already exist.

\subsection{New Concepts or Events}
For example, any events or concepts that occurred or developed after 2022 are essentially unknown to current LLMs.

\subsection{Culture Transfer}
This involves using concepts from low-resource languages.
\subsection{Construction}
Using the concepts obtained, we can input them into several pre-designed templates to generate queries. Some examples of these templates are as follows:
\begin{itemize}
    \item What is the meaning of \{concept\} (catchphrase)?
    \item What is the impact of the \{concept\} (event)?
    \item What diseases can \{concept\} be applied to (medical)?
    \item What is the symptom of \{concept\} (disease)?
    \item What can we learn from the \{concept\} (business/law cases)?
    \item ...
\end{itemize}
\section{Contributions}
\begin{itemize}
\item Our method focuses on the prevention stage, thereby preventing all potential hallucination responses.
\item Our method is not limited to a specific type of task and can be applied to open-ended conversations.
\item Our method only requires the model itself, without relying on third-party tools or models.
\item By using concept familiarity to define the hallucination level, our method offers better interpretability.
\item Our method does not require sampling techniques, resulting in robust and stable results.
\end{itemize}
